Spectroscopic and asteroseismic analysis of the remarkable main-sequence A star KIC 11145123

A spectroscopic analysis was carried out to clarify the properties of KIC 11145123 -- the first main-sequence star with a determination of core-to-surface rotation -- based on spectra observed with the High Dispersion Spectrograph (HDS) of the Subaru telescope. The atmospheric parameters ($T_{\rm eff} = 7600$ K, $\log g = 4.2$, $\xi = 3.1$ km s$^{-1}$ and $ {\rm [Fe/H]} = -0.71$ dex), the radial and rotation velocities, and elemental abundances were obtained by analysing line strengths and fitting line profiles, which were calculated with a 1D LTE model atmosphere. The main properties of KIC 11145123 are: (1) A low $ {\rm [Fe/H]} = -0.71\pm0.11$ dex and a high radial velocity of $-135.4 \pm 0.2$ km s$^{-1}$. These are remarkable among late-A stars. Our best asteroseismic models with this low [Fe/H] have slightly high helium abundance and low masses of 1.4 M$_\odot$. All of these results strongly suggest that KIC 11145123 is a Population II blue straggler; (2) The projected rotation velocity confirms the asteroseismically predicted slow rotation of the star; (3) Comparisons of abundance patterns between KIC 11145123 and Am, Ap, and blue stragglers show that KIC 11145123 is neither an Am star nor an Ap star, but has abundances consistent with a blue straggler. We conclude that the remarkably long 100-d rotation period of this star is a consequence of it being a blue straggler, but both pathways for the formation of blue stragglers -- merger and mass loss in a binary system -- pose difficulties for our understanding of the exceedingly slow rotation. In particular, we show that there is no evidence of any secondary companion star, and we put stringent limits on the possible mass of any such purported companion through the phase modulation (PM) technique.

==> Response_to_the_referee <==
Reply to the referee comment:

Dear Dr. Royer, 

Thanks a lot for your understanding of our revised version of the paper.
Following your comment on the space motion of the star, we revised the sentence to explain the space motion a bit clearer, which
is highlighted in red colour.
We assume the rotation component  of the peculiar velocity to be the observed radial velocity, and estimated the rotation
component around the Galactic centre, which is significantly slower than those of the Sun and Population I stars. 


Revision of sec 7.4.4:
......
Together those give a distance of about 1.7\,kpc. The galactic longitude of KIC\,11145123 is $81.7^{\circ}$, which means the star is nearly in the direction of galactic rotation. With the approximate distance,  it is easy to calculate that KIC\,11145123 is at about the same distance from the galactic centre as is the Sun. 
%% revised sentence:
If we assume that the observed radial velocity of KIC\,11145123 is close to the component of its peculiar velocity along the direction of Galactic rotation, given the Sun's galactic orbital velocity of 220\,km~s$^{-1}$ and its component of the peculiar velocity $V_{\odot} =$ 5.2\,km~s$^{-1}$, the large velocity of approach  of KIC\,11145123 of $-135$\,km~s$^{-1}$ shows it, therefore, to be orbiting in the direction of rotation of the Galaxy with the rotation component of  $\Theta = 90$\,km~s$^{-1}$, -- albeit much more slowly than the Sun and typical Population I stars -- indicating that it is a halo, or runaway star. 
%%
.....

Best regards,
The authors

